Investigating a Benchmark for Training-set free Evaluation of Linguistic Capabilities in Machine Reading Comprehension

Performance of NLP systems is typically evaluated by collecting a large-scale dataset by means of crowd-sourcing to train a data-driven model and evaluate it on a held-out portion of the data. This approach has been shown to suffer from spurious correlations and the lack of challenging examples that represent the diversity of natural language. Instead, we examine a framework for evaluating optimised models in training-set free setting on synthetically generated challenge sets. We find that despite the simplicity of the generation method, the data can compete with crowd-sourced datasets with regard to naturalness and lexical diversity for the purpose of evaluating the linguistic capabilities of MRC models. We conduct further experiments and show that state-of-the-art language model-based MRC systems can learn to succeed on the challenge set correctly, although, without capturing the general notion of the evaluated phenomenon.

==> figure.tex <==

\tikzset{every picture/.style={line width=0.75pt} } %set default line width to 0.75pt        
\tikzset{every node/.style={scale=0.87}}
\tikzset{
mybrace/.style={decorate,decoration={brace,aspect=#1,amplitude=5pt}}
}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,199); %set diagram left start at 0, and has height of 199

%Shape: Rectangle [id:dp12066761468185846] 
\draw   (0,0) -- (\columnwidth,0) -- (\columnwidth,205) -- (0, 205) -- cycle ;
\draw   (0,176) -- (\columnwidth,176) ;
% \draw   (416,80) -- (670,80) -- (670,131) -- (416,131) -- cycle ;
\draw  [dashed] (10,33) -- (290,33);
%\draw [decorate,decoration={brace,amplitude=5pt,raise=0pt},xshift=0,yshift=0pt] (10,129) -- (10,3);
\draw [mybrace=0.5] (8,128) -- (8,18);
%\draw [mybrace=0.07] (207,22) --  (207,140);
% Text Node
\draw (4,0) node [anchor=north west][inner sep=0.5pt]  [font=\normalsize] [align=left] {\textbf{P:} \emph{\Circled{1} In the beginning of the match \textcolor[rgb]{0.29,0.56,0.89}{\underline{Alice Jameson}}... }};
% Text Node
\draw (10,19) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(C) Original}: \emph{scored}};
% Text Node
\draw (10,35) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(I1) Modal negation}: \emph{\emph{\textcolor[rgb]{0.82,0.01,0.11}{couldn't curl}} in}};
% Text Node
\draw (10,51) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(I2) Adverbial Modification}: \emph{\textcolor[rgb]{0.82,0.01,0.11}{\emph{almost}} scored}};
% Text Node
\draw (10,67) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(I3) Implicit Negation}: \emph{\textcolor[rgb]{0.82,0.01,0.11}{\emph{was prevented from}} curling in}};
% Text Node 
\draw (10,83) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(I4) Explicit Negation}: \emph{\textcolor[rgb]{0.82,0.01,0.11}{\emph{didn't succeed in}} curling in}};
% Text Node
\draw (10,99) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=center] { \textbf{(I5) Polarity Reversing VP}: \emph{\textcolor[rgb]{0.82,0.01,0.11}{\emph{lacked the nerve to}} score}};
% Text Node
\draw (10,115) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=left] { \textbf{(I6) Explicit Neg. VP}: \textcolor[rgb]{0.82,0.01,0.11}{didn't get the chance to} \emph{score}};
% Text Node
\draw (5,131) node [anchor=north west][inner sep=0pt]  [font=\normalsize\itshape] [align=left] {\textbox{ ...a goal from 26 metres away following run through the centre. \Circled{2} Then \textcolor[rgb]{0.25,0.46,0.02}{\underline{Anne Thomson}} retaliated quickly when she slotted in a wonderful goal [...] }};
% Text Node
\draw (0,178) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=left] {{ \textbf{Q:} \emph{Who scored the first goal?}}};
% Text Node
\draw (0,192) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=left] {{ \textbf{A:} \textcolor[rgb]{0.29,0.56,0.89}{Alice Jameson}}};
% Text Node
\draw (125,192) node [anchor=north west][inner sep=0pt]  [font=\normalsize] [align=left] {{ \textbf{A with \textcolor[rgb]{0.82,0.01,0.11}{SAM}:} \textcolor[rgb]{0.25,0.46,0.02}{Anne Thomson}}};

\end{tikzpicture}

% \begin{table}[t]
%     \centering
%     \begin{tabularx}{1\columnwidth}{|X|}
%     \hline
%     \textbf{Original Context: } \emph{After the kickoff {\color{blue}\emph{Despina Daniell}} scored a goal from 26 metres away after a decisive counter-attack. Then {\color{green}\emph{Anne Thomson}} added more insult to the injury when she slotted in a goal from Linda Burger 's soft clearance [\ldots] }  \\
    
%     \textbf{Modal Negation:} \emph{After the kickoff Despina Daniell {\color{red} couldn't}
%     score a goal from 26 metres away after a decisive counter-attack. [\ldots] } \\ 
%     \textbf{Adverbial Modification:} \emph{After the kickoff Despina Daniell {\color{red} almost}
%     scored a goal from 26 metres away after a decisive counter-attack. [\ldots] } \\
%     \textbf{Verbs of Implicit Negation:} \emph{After the kickoff Despina Daniell {\color{red} was prevented from} curling in a goal from 26 metres away after a decisive counter-attack. [\ldots] } \\
%     \textbf{Explicitly negated Verbs:} \emph{After the kickoff Despina Daniell {\color{red} didn't succeed in} curling in a goal from 26 metres away after a decisive counter-attack. [\ldots] } \\
%     \textbf{Polarity reversing Expressions:} \emph{After the kickoff Despina Daniell {\color{red} lacked the nerve} to
%     score a goal from 26 metres away after a decisive counter-attack.[\ldots] } \\
    
%     \textbf{Negated polarity preserving Expressions:} \emph{After the kickoff Despina Daniell {\color{red} wouldn't find the opportunity} to
%     score a goal from 26 metres away after a decisive counter-attack.[\ldots] } \\
%     \hline
%     \textbf{Question}: \emph{Who scored the first goal of the match?} \\
%     \hline
%     \end{tabularx}
%     \caption{Chosen SAM categories. Is it better to have a sort of flow diagram here?}
    
%     \label{tab:SAM}
% \end{table}
% contribute to the “at issue” content of the utterance in which they ap-pear vs. those that do not 
